Out-of-Distribution Data: An Acquaintance of Adversarial Examples -- A Survey

Deep neural networks (DNNs) deployed in real-world applications can encounter out-of-distribution (OOD) data and adversarial examples. These represent distinct forms of distributional shifts that can significantly impact DNNs' reliability and robustness. Traditionally, research has addressed OOD detection and adversarial robustness as separate challenges. This survey focuses on the intersection of these two areas, examining how the research community has investigated them together. Consequently, we identify two key research directions: robust OOD detection and unified robustness. Robust OOD detection aims to differentiate between in-distribution (ID) data and OOD data, even when they are adversarially manipulated to deceive the OOD detector. Unified robustness seeks a single approach to make DNNs robust against both adversarial attacks and OOD inputs. Accordingly, first, we establish a taxonomy based on the concept of distributional shifts. This framework clarifies how robust OOD detection and unified robustness relate to other research areas addressing distributional shifts, such as OOD detection, open set recognition, and anomaly detection. Subsequently, we review existing work on robust OOD detection and unified robustness. Finally, we highlight the limitations of the existing work and propose promising research directions that explore adversarial and OOD inputs within a unified framework.

==> related_work.tex <==
\section{Related Work}

\subsection{Out-of-Distribution Detection}

Early work in post-hoc OOD detection mainly relies on softmax score which tends to become overconfident about samples which are far away from the training distributions. Hence, Liu et al.~\cite{energy} introduce a score based on the energy of a prediction to mitigate the failures of the softmax score. The paper uses the logits predicted by a classifier to compute the free energy score of a sample to better distinguish OOD samples from in-distribution data. The free energy of a sample $x$ is defined as,
\begin{equation}
\label{eq:freeenergy}
    E(x;f) = -T\cdot \log\sum_{i}^{K} e^{f_i(x)/T}
\end{equation}
where $T$ is the temperature parameter and $K$ is the number of classes of classifier $f$. Here, the energy score can be considered as a generalised version of the softmax score. The paper shows that the softmax score is a special case of the energy function where all the logits are shifted by their maximum value. During inference, in-distribution data has a higher negative energy score compared to OOD data. Hence, a threshold ($\tau$) is chosen for OOD detection such that a high fraction of inputs is correctly distinguished by the energy score. Thus, an energy based OOD detector can be expressed as,
\begin{equation}
    G(x;\tau,f) = \begin{cases} 
 0 & \text{if $-E(x;f) \leq \tau$} \\  
 1 & \text{if $-E(x;f) > \tau$}   
 \end{cases} 
\end{equation}

In post-hoc OOD detection, the energy gap might not always be optimal to distinguish between in and out-of-distribution data. Hence, this work proposes an energy bounded learning objective as well. Here, the classifier is fine tuned to explicitly create an energy gap between in and out-of-distribution samples by assigning lower energies for in-distribution data and higher energies for out-of-distribution data. This is achieved by adding an energy regularisation term to the training objective as follows:
\begin{equation}
\label{eq:energy_objective}
    \min_{\theta} \quad \mathbb{E}_{(x,y) \sim {\mathcal{D}_{\text{in}}^{\text{train}}}} [-\log F_y(x)] + \lambda\cdot L_{\text{energy}}  
\end{equation} 
where $F(x)$ is the softmax output of the classifier and $\mathcal{D}_{\text{in}}^{\text{train}}$ is the in-distribution training data. The first term in Equation~\ref{eq:energy_objective} is the standard cross entropy loss while the second energy-based term consists of two squared hinge loss terms with separate margin hyper parameters for in and out-of-distribution data. Simply put, the classifier penalises both in-distribution data having higher energies than the specified in-distribution margin as well as out-of-distribution data having lower energies than the specified out-of-distribution margin. This allows a greater flexibility in shaping the energy surface to further differentiate the energies between in and out-of-distribution data.     

The authors evaluate the proposed methods on standard benchmark datasets using the false positive rate of OOD samples when true positive rate of in-distribution samples is at 95\% (FPR95), and show that energy score reduces the average FPR95 by 18.03\% compared to the softmax baseline~\cite{softmaxscore} on CIFAR-10 for post-hoc OOD detection. Furthermore, the energy fine-tuned model reduces the FPR95 by 5.20\% on CIFAR-10 compared to Outlier Exposure~\cite{outlierexposure}. 

\textbf{****************************************************}

As an extension of ~\cite{energy}, Morteza et al.~\cite{gem_score} leverage the knowledge of Mahalanobis distance~\cite{mahalanobis1936generalized} to modify the free energy function such that the energy score is proportional to the data density. By modelling the feature space as a class-conditional multivariate Gaussian distribution, this paper introduces a novel scoring function named \textit{GEM} (Gaussian mixture based Energy Measurement) based on the Gaussian generative model. Furthermore, the paper provides a unified theoretical framework that characterises the interpretations of existing OOD scoring functions such as softmax~\cite{softmaxscore} and maximum Mahalanobis  distance~\cite{mahalanobis}. 

The theoretical framework is based on the assumption that the in-distribution data is drawn from class-conditional Gaussian distributions. Hence, the probability density of class $y_i \in \mathcal{Y}$ can be modelled as,
\begin{equation}
    x|y_i \sim \mathcal{N}(\mu_i,\Sigma)
\end{equation}
where $\mathcal{Y}$ is the label space, $\mu_i\in\mathbb{R}^d$ is the mean of class $i$ and $\Sigma \in \mathbb{R}^{d\times d}$ is the covariance matrix. Here $d$ is the dimension of the input space $\mathcal{X}$ where $x \in \mathcal{X}$.
% Let the input space be $\mathcal{X}$ and $\mathcal{P}_{\mathcal{X},\mathcal{Y}}^{\text{in}}$ denote a probability distribution defined on $\mathcal{X} \times \mathcal{Y}$. 
Thus, class conditional density can be defined as,
\begin{equation}
    \mathcal{P}_{\mathcal{X}|\mathcal{Y}}^{\text{in}} (x|y_i) = \frac{\exp(-\frac{1}{2}(x-\mu_i)^{\top}\Sigma^{-1}(x-\mu_i))}{\sqrt{(2\pi)^d|\Sigma|}} 
\end{equation}
Consequently, the input data distribution can be formulated as the summation of the class conditional densities as in Equation~\ref{eq:inputdist}.
\begin{equation}
    \label{eq:inputdist}
    \mathcal{P}_{\mathcal{X}}^{\text{in}}(x) = \sum_{j=1}^{K} \mathcal{P}_{\mathcal{X}|\mathcal{Y}}^{\text{in}} (x|y_j) \cdot \mathcal{P}_{\mathcal{Y}}^{\text{in}}(y_j)
\end{equation}
Here $\mathcal{P}_{\mathcal{Y}}^{\text{in}}(y_j)$ is the prior probability of class $y_j$. Note that for convenience, here we consider the equal prior case (i.e. $\forall y_j \in \mathcal{Y}$;  $\mathcal{P}_{\mathcal{Y}}^{\text{in}}(y_j) = \frac{1}{K}$). However, the analysis holds for the unequal prior scenario as well. The intuition behind an ideal OOD detector is to be proportional to the data density. The authors show that existing scoring functions such as Maximum Softmax Probability and Maximum Mahalanobis distance are not aligned with the true density, thus becoming sub optimal. As a solution, the GEM score is introduced by replacing the model $f$ in free energy equation~\ref{eq:freeenergy} by Mahalanobis distance from the input $x$ to each class distributions as follows.
\begin{equation}
    \label{gemscore}
    \begin{split}
    \text{GEM}(f,x) &= \log\sum_{j=1}^{K}\exp(-\frac{1}{2}(x-\mu_j)^{\top}\Sigma^{-1}(x-\mu_j)) \\
    & \propto \log\mathcal{P}_{\mathcal{X}}^{\text{in}}(x)
    \end{split}
\end{equation}
As shown in Equation~\ref{gemscore}, GEM score is a special case of negative free energy, where instead of directly using logits $f_j(x)$, the exponent takes the form of Mahalanobis distance. As one of the main contributions, this paper provides provable guarantees for OOD detection which is often missing in literature. 

\textbf{****************************************************}

Wei et al.~\cite{logitnormalization} relate the problem of models being over-confident on both in and out-of-distribution data to the norm of the logits and introduce a simple fix to the cross-entropy loss. The paper argues that the norm of the logits keeps increasing during training which eventually ends up in overconfident outputs. Hence, as the solution, a novel technique called \textit{Logit Normalization} a.k.a. \textit{LogitNorm} is introduced to decouple the influence of the logit norm during model optimization. The idea behind Logit Normalization is to enforce a constant norm on the logit vector that is the output prior to the ultimate softmax layer.  

LogitNorm is motivated by the fact that even when a majority of training samples are correctly classified, the cross-entropy loss along with softmax continues to increase the magnitude of the logits thus resulting in overconfidence despite having no improvement in model accuracy. Consequently, LogitNorm decouples the effect of the norm of the output from the training objective and its optimization by normalising the logit vector to have a constant norm during training. This simple fix tends to produce distinguishable softmax scores between in and out-of-distribution inputs. The modified objective function takes the following form.
\begin{equation}
\begin{aligned}
    &\text{minimize} \quad  \mathbb{E}_{\mathcal{P}_ {\mathcal{XY}}}[\mathcal{L_{\text{CE}}}(f(x;\theta),y)] \\
    & \text{subject to} \quad ||f(x;\theta)||_2 = \alpha
\end{aligned}
\end{equation}
Here, $\mathcal{L}_{\text{CE}}$ is the cross-entropy loss between the logits $f(x;\theta)$ and the ground truth $y$ and $\alpha$ is a constant. As solving a constrained optimization is non-trivial in the context of modern neural networks, the authors convert this objective into an alternative loss function which is end-to-end trainable. First, the logit vector $f$ is decomposed into two components:
\begin{equation}
    f = ||f|| \cdot \hat{f},
\end{equation}
where $||f||$ is the Euclidean norm or the magnitude of $f$ and $\hat{f}$ is the unit vector in the same direction as $f$. LogitNorm encourages $\hat{f}$ to be consistent with the corresponding one-hot encoded label, without optimizing $||f||$. Hence, it normalises the logit vector as a unit vector with a constant magnitude. The softmax cross-entropy is then applied on the normalised logit vector instead of the original logits. The modified loss function is defined as:
\begin{equation}
    \mathcal{L}_{\text{logit\_norm}}(f(x;\theta),y) = -\log\frac{e^{f_y/(\tau ||f||)}}{\sum_{i=1}^{k} e^{f_i/(\tau ||f||)}}
\end{equation}
where $\tau$ is the temperature parameter which regulates the magnitude of the logits. This idea is equivalent to having an input dependent temperature unlike in distillation~\cite{distillation} where the temperature is constant for all inputs. Extensive experiments on common benchmarks show that LogitNorm reduces the average FPR95 by up to 42.3\%. 

\textbf{****************************************************}

Existing score-based OOD detectors depend solely on a single source which can either be the features, the logits or the softmax probabilities of a given input. Wang et al.~\cite{virtuallogitmatching} combines the information from the feature space and the logit space to create a virtual OOD class to study the influence of the lost information going from features to logits. The probability of this virtual class is used to quantify the OOD-ness of a sample, which is termed as the \textit{Virtual-logit Matching} (ViM) score. The intuition behind ViM is that performance of existing OOD score functions is limited as they are restricted to a single information source. That is, using only features disregards the model parameters with class-dependent information while using only logits or probabilities ignores class-agnostic feature components in the null space. Hence, the ViM score computes the residual of the features against a principal subspace and constructs a virtual OOD class whose logit is jointly determined by the existing logits and the input features. 

Consider a $K$-class classifier that transforms input features $x \in \mathbb{R}^N$ into logits $l \in \mathbb{R}^K$ by a fully connected layer with weight $W \in \mathbb{R}^{N \times K}$ and bias $b \in \mathbb{R}^K$, $i.e. \ l = W^Tx + b$. ViM first shifts the feature space by a vector $o = -(W^T)^+b$, where $(.)^+$ is the Moore-Penrose pseudo inverse, to make the logit computation free from the bias. Then the principal subspace $P$ is defined with respect to the training set $X$ whose rows are the shifted features. Let the eigendecomposition on $X^TX$ be,
\begin{equation}
    X^TX = Q \Lambda Q^{-1}
\end{equation}
with eigenvalues in $\Lambda$ sorted in descending order. Then $P$ is the $D$-dimensional subspace spanned by the eigenvectors of the largest $D$ eigenvalues of $X^TX$ (i.e. the first $D$ columns of $Q$). The residual $x^{P^{\bot}}$ is the projection of $x$ onto $P^{\bot}$ which is the null space of $P$ and is computed as,
\begin{equation}
    x^{P^{\bot}} = RR^Tx
\end{equation}
where $R \in \mathbb{R}^{N \times (N-D)}$ is the last $N-D$ columns of $Q$. Then, the virtual logit is computed by re-scaling the norm of the residual with a model-based constant $\alpha$. Since, softmax normalization is highly sensitive to the scale of logits, $\alpha$ matches the scale of the virtual logits with that of the original logits as in Equation~\ref{eq:virtuallogit}.
\begin{equation}
    \label{eq:virtuallogit}
    l_0 = \alpha||x^{P^{\bot}}|| = \alpha\sqrt{x^TRR^Tx}
\end{equation}
\begin{equation*}
    \alpha = \frac{\sum_{i=1}^{n} \max_{j=1,\dots,K}\{l_{j}^{i}\}}{\sum_{i=1}^{n}||x_{i}^{P^{\bot}}||}
\end{equation*}
Here, $x_1,x_2,\dots,x_n$ are uniformly sampled $n$ training samples and $l_j^i$ is the $j$-th logit of $x_i$. The numerator of $\alpha$ corresponds to the mean of the maximum logits while the denominator represents the average norm of the virtual logit on the training set. Therefore, re-scaling the norm of the residual using $\alpha$ ensures that the virtual logit is in the same scale as the maximum of the original logits. 

Finally, the computed virtual logit is appended to the original $K$ logits ($l_i$) to compute the softmax scores for each class. The probability score of the virtual OOD class is the ViM score as in Equation~\ref{eq:vimscore}.
\begin{equation}
\label{eq:vimscore}
    \text{ViM}(x) = \frac{e^{\alpha\sqrt{x^TRR^Tx}}}{\sum_{i-1}^{K}e^{l_i} + \alpha\sqrt{x^TRR^Tx}}
\end{equation}
This equation shows that if the norm of the residual of an input is larger than its original logits, then it is highly likely to be OOD, and vice versa.  

\textbf{****************************************************}

The work by Huang et al.~\cite{gradnorm} explores the gradient space for detecting OOD samples and introduces a method named \textit{GradNorm} which employs the vector norm of gradients of model parameters. Here, the gradients are computed by back-propagating the Kullback-Leibler (KL) divergence loss between the softmax output and a uniform probability distribution. KL divergence quantifies the closeness of two distributions. Therefore, the intuition behind using KL divergence with a uniform distribution is that the predictions for in-distribution data tend to concentrate on one class (i.e. the ground-truth class), resulting in a higher deviation from a uniform distribution. Consequently, in-distribution data will have larger KL divergence compared to OOD data as the predictions for OOD samples, are much closer to a uniform distribution. 

Let the model-predicted probability distribution be $q=\{q_i\}$ and a reference probability distribution be $p=\{p_i\}$. Then the KL divergence between $p$ and $q$ is formally defined as,
\begin{equation}
\label{eq:kldiv}
\begin{aligned}
    D_{\text{KL}}(p\ ||\ q) &= \sum_ip_i \log\frac{p_i}{q_i} \\
    &= -\sum_i p_i \log q_i + \sum_i p_i\log p_i \\
    &= H(p,q) - H(p)
\end{aligned}
\end{equation}
Here $H(p,q)$ refers to the cross-entropy between $p$ and $q$, and $H(p)$ refers to the entropy of $p$. In GradNorm, $p$ is set to be a uniform distribution $u = [1/K,1/K,\dots,1/K] \in \mathbb{R}^C$ and $q$ is the softmax output of the model. Then Equation~\ref{eq:kldiv} becomes,
\begin{equation}
\label{eq:gradnormkl}
    D_{\text{KL}}(u\ ||\ \text{softmax}(f(x))) = -\frac{1}{K}\sum_{i=1}^{K} \log \frac{e^{f_i(x)/T}}{\sum_{j=1}^K e^{f_j(x)/T}} - H(u)
\end{equation}
The first term represents the cross-entropy loss between the softmax output and the uniform vector and the second term is the entropy of the uniform vector which is a constant. The GradNorm OOD score is now defined via a vector norm of gradients of the KL divergence loss defined in Equation~\ref{eq:gradnormkl} with respect to a set of selected parameters $w$ as,
\begin{equation}
    S(x) = ||\frac{\partial D_{\text{KL}}(u\ ||\ \text{softmax}(f(x)))}{\partial w}||_p
\end{equation}
where $||.||_p$ denotes the $L_p$ norm. As discussed earlier, softmax output for in-distribution data tends to have a higher KL divergence with respect to a uniform distribution, thus resulting in higher gradient norms. In contrast, as the predictions for OOD data will be distributed approximately uniformly among the classes, the KL divergence will be much smaller resulting in smaller gradient norms. Hence, OOD detection can be done by selecting a threshold such that a majority of in-distribution samples are correctly classified (i.e. 95\% true postive rate).

The standard cross-entropy loss can be viewed as the KL-divergence between the softmax output and the one-hot encoded ground-truth for a given input. Instead, GradNorm employs the KL divergence with a uniform target as it offers two main advantages over the standard cross-entropy loss. First, GradNorm does not require any ground-truth label (i.e. \textit{label-agnostic}), hence can be flexibly used even in absence of the ground-truth for both in-distribution and OOD data during inference. Secondly, GradNorm captures the uncertainty of all classes providing more information for detecting OOD samples. Empirical results on OOD detection benchmark datasets show that GradNorm outperforms then previous best method~\cite{energy}, reducing the average FPR95 by up to 16.33\%.  

\textbf{****************************************************}

Inspired by Intergral Probability Metrics (IPMs)~\cite{IPM}, Dong et al. introduce a technique called \textit{Neural Mean Discrepancy} (NMD)~\cite{neuralmeandisc} which differentiates OOD data from in-distribution data using the mean of the model activations (i.e. \textit{Neural Mean}). The authors argue that standard off-the-shelf models already contain sufficient information on training distribution which can be leveraged to detect OOD samples. On that account, NMD employs the difference between the neural means of training data and OOD data for reliable OOD detection. This method is computationally efficient as well as it only requires a forward pass followed by a lightweight classifier which can be a simple logistic regression or MLP model. Furthermore, in the presence of BatchNormalization layers, neural mean of training data can be extracted without any computations.

In order to understand the math behind NMD, it is beneficial to have a simple understanding about IPMs. IPMs are a family of probability distance measures defined on two distributions $\mathcal{P}$ and $\mathcal{Q}$. Let $\mathcal{D}_{\text{tr}}$ be the training set from the in-distribution $\mathcal{P}$, and $\mathcal{I}$ be a given batch of input examples from an unknown distribution $\mathcal{Q}$. Then IPMs can be defined as,
\begin{equation*}
\label{eq:ipm}
    \begin{split}
        \text{IPM}_{\mathcal{F}}(\mathcal{Q},\mathcal{P}) &= \sup_{\varphi \in \mathcal{F}} (\mathbb{E}_{x \sim \mathcal{Q}}[\varphi(x)] - \mathbb{E}_{s \sim \mathcal{P}}[\varphi(s)]) \\
        &= \sup_{\varphi \in \mathcal{F}} \Bigg( \frac{1}{|\mathcal{I}|} \sum_{i=1}^{|\mathcal{I}|} \varphi(x_i) - \frac{1}{|\mathcal{D}_{\text{tr}}|} \sum_{j=1}^{|\mathcal{D}_{\text{tr}}|} \varphi(s_j)\Bigg), 
    \end{split}
\end{equation*}
where $\varphi(.)$ denotes the witness function which projects the inputs to a new space. Then the means of the two projected sets are compared to measure the distance between the two distributions $\mathcal{P}$ and $\mathcal{Q}$. In NMD, rather than explicitly defining $\varphi$, the authors use channels in the off-the-shelf model as the witness function. This is justified by the relaxation of the supremum in Equation~\ref{eq:ipm} in the context of OOD detection, assuming that as long as a function is capable of differentiating the statistics such as mean of samples in the projected space between in and out-of-distribution data, that function is qualified to be a witness function. Hence, NMD is computed by taking a certain channel $c$ in the $l$-th layer of the model as the witness function $f_c^l$ as follows.
\begin{equation}
\label{eq:nmd}
    \begin{aligned}
        \text{NMD}_c^l(\mathcal{I}) &= \frac{1}{|\mathcal{I}|\cdot d^2} \sum_{i=1}^{|\mathcal{I}|} \sum_{m=1}^d \sum_{n=1}^d f_c^l(x_i)_{m,n} \\
        &- \frac{1}{|\mathcal{D}_{\text{tr}}|\cdot d^2} \sum_{j=1}^{|\mathcal{D}_{\text{tr}}|} \sum_{m=1}^d \sum_{n=1}^d f_c^l(s_j)_{m,n} \\
        &= \mu[f_c^l(\mathcal{I})] - \mu[f_c^l(\mathcal{D}_{\text{tr}})] 
    \end{aligned}
\end{equation}
Here, $d$ is the spacial size the activation maps. To further improve the performance, the authors combine NMDs from all channels across all layers in the model and construct a $C$-dimensional NMD vector where $C$ is the total number of channels in $L$ layers of the model. Thus, for a given input batch $\mathcal{I}$, the NMD vector can be formally defined as follows.
\begin{equation}
\scriptsize
    \text{NMD}(I) = \{\text{NMD}_1^1, \text{NMD}_2^1,\dots, \text{NMD}_1^l, \text{NMD}_2^l,\dots, \text{NMD}_1^L, \text{NMD}_2^L,\dots\} 
\end{equation}
As the receptive field increases along the depth of a model, combining NMDs from all layers captures both high-level and low-level semantics. One major drawback of IPMs for OOD detection is that they require input batches as shown in Equation~\ref{eq:nmd}. However, a practical OOD detector should be able to distinguish individual samples. Therefore, NMD employs a lightweight classifier such as a simple logistic regression or MLP model as the second stage of OOD detection. This classifier is trained using $\{(\text{NMD}(x_{\text{ID}}),0),\dots,(\text{NMD}(x_{\text{OOD}}),1)\}$ pairs and it facilitates individual predictions of unknown inputs during testing. 

Extensive experiments have been conducted using standard off-the-shelf models such as ConvNet, ResNet, VGG etc. and standard benchmark datasets such as CIFAR-10, CIFAR-100, SVHN etc. to empirically prove the performance of NMD. Moreover, to accommodate real-world OOD detection scenarios, the authors simulate different cases such as \textit{Full access}, \textit{Few-shot}, \textit{Zero-shot}, and \textit{Transfer learning} based on the amount of accessible OOD samples.  

\textbf{****************************************************}

The work by Sun et al.~\cite{react},~\cite{dice} use the activations of the penultimate layer to improve the separability of ID and OOD data. 

\cite{dice} focuses on a method named \textit{\textbf{Di}rected \textbf{S}parsification} (\textbf{DICE}) that prunes away the noisy activations to reduce the variance of the output for OOD data. This results in a sharper output distribution for OOD data making them more separable from ID data. The model predictions for ID data mostly rely on a subset of important activations compared to OOD data. DICE leverages this observation for OOD detection by ranking the weights based on their contribution and selectively using the most contributing weights (i.e., weight sparsification). The authors also provide a theoretical analysis to verify that weight sparsification reduces the output variance for both ID and OOD data. However, as OOD data consists of more noisy signals, the effect on OOD data is much higher than on ID data, thus increasing the separability between the two. 

For an input $x \in \mathcal{D}$, let the feature vector from the penultimate layer be $h(x) \in \mathbb{R}^m$. A weight vector $W\in\mathbb{R}^{m \times C}$ connects $h(x)$ to the output space with $C$ classes. The authors first define a contribution matrix $V \in\mathbb{R}^{m \times C}$ where each column $v_c \in \mathbb{R}^m$ in $V$ is defined as follows.
\begin{equation}
    v_c = \mathbb{E}_{x \in \mathcal{D}}[w_c \odot h(x)]
\end{equation}
Here, $\odot$ indicates the element-wise multiplication and $w_c$ indicates the weight vector for each class $c$. 

\textcolor{red}{TBC}


\subsection{Concurrent Detection of Adversarial and OOD inputs}

\cite{ood_adv_1} focuses on detecting adversarial and OOD inputs concurrently by leveraging the gradients w.r.t the parameters (i.e. weights and biases). A major limitation of using gradients for adversarial or OOD detection is the lack of availability of ground truth labels during inference for gradient computations. As a solution, this work utilizes a confounding label the model has not seen during training. The authors use the union of the one-hot encodings of all classes (i.e., a vector of all 1's) as the confounding label along with the binary cross-entropy loss to compute gradients. Then layer-wise gradients are used as features to be fed to a secondary classifier to detect adversarial and OOD inputs. Here, the authors define a term named \textit{effective expressivity} as the representational power of a model based on the training data and use the back-propagated gradients to study the effective expressivity of a trained model. They perceive the gradients as the amount of changes required by the model to correctly represent a given input. Hence, a larger gradient implies an input is highly unfamiliar to the model. As an OOD detector, this method is more suitable for far OOD detection than near OOD detection.

\subsection{Robust OOD Detection}

\cite{nearoodvulnerability} shows that some of the existing baselines which perform well in detecting near OOD inputs, drastically fail under adversarial perturbations. The paper focuses on CIFAR-100 (ID) vs CIFAR-10 (OOD) near OOD detection problem and show that even simple attacks such as FGSM~\cite{fgsm} can drop the AUROC performance of Mahalanobis Distance (MD) method~\cite{mahalanobis} by $\approx$57\%. As a solution, the authors show that \textit{Relative Mahalanobis Distance} (RMD) can be used as a robust OOD detector to handle near OOD inputs better. Let $z'$ be the low dimensional representation from the second to last layer of a neural network for a given test input $x'$. Then RMD is defined as,
\begin{equation}
    RMD_k(z') = MD_k(z') - MD_0(z')
\end{equation}
where $MD_k(z')$ represents the Mahalanobis distance to the class specific Gaussian distribution of class $k$ and $MD_0(z')$ indicates the Mahalanobis distance to a Gaussian distribution fitted to the entire in-distribution dataset.

It is important to note that this work uses the gradients of the \textit{OOD score} with respect to the input to conduct FGSM attacks instead of the gradients of the loss with respect to the input. This paper reports that regardless how expressive the embeddings generated by powerful networks such as Vision Transformers (ViT) are, they still are susceptible against near OOD adversarial examples. Furthermore, the authors empirically show that working with lower resolution images and OOD score ensembles (i.e., Average of OOD scores from two well performing  models fine-tuned on CIFAR-100) increase the adversarial robustness. 

\textbf{****************************************************}

Even though the standard method of evaluating the performance of an OOD detector is via AUROC scores relative to specific OOD datasets (e.g., CIFAR10 vs SVHN), this ponders the question of whether we will be able to achieve the same performance across all other real world OOD data. To tackle this problem, Yoon et al. \cite{detector_evaluator} have proposed a method, Evaluation-via-Generation (EvG), to evaluate the performance of an OOD detector. The method consists of a variation model that performs affine transformations, color jittering, or creating new data points by recombining existing OOD data using a GAN. An adversarial distribution for a single sample is then defined as
\begin{equation}
p_f(z) = \frac{1}{Z} exp(-f(gz)/T),\ Z=\int _\mathcal{Z}exp(-f(gz)/T)dz< \infty
\end{equation}

where $g(z)$ is a generator used to augment OOD data utilizing existing OOD data with the parameters $z \in \mathcal{Z}$ (e.g., for the affine transform $z$ = [35, -10, 15], corresponding to the rotation angle, translation on the x-axis and shear amount respectively), $f$ is an OOD detector function that outputs a high value for OOD data, and $T$ is the temperature. The distribution can be seen as an energy-based model where $f(x)$ serves as energy. A Markov Chain Monte Carlo (MCMC) optimization algorithm is then used to draw out a sample from this distribution with the lowest detector score, which would be the most challenging OOD sample for the detector.

AUROC scores obtained by evaluating the OOD detectors with samples obtained from the above process show that some of the robust OOD detectors (AUROC$>$0.9) did not perform well compared to their performance on unaugmented data. The authors additionally introduce a new metric to evaluate OOD detectors by calculating the rank of the smallest detection score (score from the worst performing OOD sample, i.e.; the OOD sample considered the closest to ID) obtained from the OOD data with respect to the scores of the in-distribution data.


\textbf{****************************************************}

\cite{atd} presents a strong detector of OOD inputs even when they are perturbed by adversarial threat models. The existing work on robust OOD detection has not been end-to-end (i.e., the attack is done on the classification model to evaluate the OOD detector). This paper bridges that gap by evaluating OOD detectors with an end-to-end attack and show that almost all the previous methods perform worse than a random classifier. Subsequently, the authors propose a robust model named \textit{Adversarially Trained Discriminator} (ATD) that uses a GAN-based method to generate OOD samples and differentiate them from the in-distribution samples (closed set). At the same time, the authors conduct adversarial training on the closed set and a small open set to achieve robustness on them as well. Hence, ATD achieves robustness from two aspects as follows.
\begin{itemize}
    \item Implicit robustness for a wide range of OOD inputs via the Generator
    \item Robustness via adversarial training using perturbed ID and OOD data. 
\end{itemize}
The resultant Discriminator is shown to outperform the previous methods by a significant margin. It is important to note that only samples from the closed and open sets are perturbed in adversarial training. The samples generated from the Generator are not perturbed as it would make the training of the GAN unstable. Furthermore, this GAN generates and discriminates low-dimensional features instead of images as it is easier to bring the Generator to the ideal case than working with high-dimensional images. 

\subsection{Adversarial Robustness via Domain Generalization/Adaptation}

Different adversarial attacks come from different distributions. Hence, domain generalization techniques in OOD context can be used to improve the adversarial robustness of neural networks. Here, the different domains are attacks such as PGD, CW, and AutoAttack. The work done by Ibrahim et al.~\cite{rex} leverage the idea of Variance-based Risk Extrapolation (REx) to improve the adversarial robustness against multiple attacks seen during training and testing times. REx adds the variance of the Empirical Risk Minimization (ERM) loss across different domains (i.e., adversarial attacks) as a loss penalty. This encourages worst-case robustness over more extreme versions of the shifts observed between training domains (i.e, in this case more powerful adversarial attacks). 

The authors sets as the baseline, the robustness achieved by adversarial training with both individual attacks such as $PGD_{\infty}$, $PGD_2$, $PGD_1$, $CW_2$, $AutoAttack$ etc. as well as their ensembles. Then for the multi-attack scenarios, the term that penalizes the variance of the domains is added to achieve further robustness. Experiments on MNIST and CIFAR10 shows that REx improves the performance of all baselines against an ensemble of attacks, by sacrificing a little robustness against the weakest individual attacks.

\textbf{****************************************************}




